Pro3D-Editor : A Progressive-Views Perspective for Consistent and Precise 3D Editing

Text-guided 3D editing aims to precisely edit semantically relevant local 3D regions, which has significant potential for various practical applications ranging from 3D games to film production. Existing methods typically follow a view-indiscriminate paradigm: editing 2D views indiscriminately and projecting them back into 3D space. However, they overlook the different cross-view interdependencies, resulting in inconsistent multi-view editing. In this study, we argue that ideal consistent 3D editing can be achieved through a \textit{progressive-views paradigm}, which propagates editing semantics from the editing-salient view to other editing-sparse views. Specifically, we propose \textit{Pro3D-Editor}, a novel framework, which mainly includes Primary-view Sampler, Key-view Render, and Full-view Refiner. Primary-view Sampler dynamically samples and edits the most editing-salient view as the primary view. Key-view Render accurately propagates editing semantics from the primary view to other key views through its Mixture-of-View-Experts Low-Rank Adaption (MoVE-LoRA). Full-view Refiner edits and refines the 3D object based on the edited multi-views. Extensive experiments demonstrate that our method outperforms existing methods in editing accuracy and spatial consistency.

==> table/compare.tex <==
\begin{table}[!t]
\caption{\textbf{Parameter comparison} of our method and existing methods. While our fine-tuning approach leads to higher GPU memory and time costs than 
existing training-free methods, it enables semantically relevant local 3D editing, which existing methods cannot achieve.}
\centering
\begin{tabularx}{\textwidth}{>{\centering\arraybackslash}m{2cm}>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\toprule
Method & View Resolution & Editing Time & GPU Memory Usage \\ 
\midrule
Tailor3D & 448 $\times$ 448 & 4 min & 65 GB \\
LGM & 256 $\times$ 256 & 5 sec & 10 GB \\
MVEdit & 512 $\times$ 512 & 6 min & 13 GB  \\
3DAdapter & 512 $\times$ 512 & 10 min & - \\
\midrule
\textbf{\textit{Pro3D-Editor}} & 768 $\times$ 768 & 90 min & 60 GB \\
\bottomrule
\end{tabularx}
\label{tab:ablation_all}
\vspace{-4mm}
\end{table}


==> table/comparison3D.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|ccc}
\toprule
Method &  Text-Asset Alignment & 3D Plausibility & Textual Details \\ 
\midrule
Tailor3D & 50\% & 56\% & 61\%  \\
MVEdit & 54\% & 78\% & 48\%  \\
3D-Adapter & 95\% & 98\% & 88\%  \\
LGM & 79\% & 70\% & 75\% \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison using GPTEval3D}.}
\label{tab:comparison3d}
\end{table}

